How quickly can you pack short paths? Engineering a search-tree algorithm for disjoint s-t paths of bounded length

We study the Short Path Packing problem which asks, given a graph $G$, integers $k$ and $\ell$, and vertices $s$ and $t$, whether there exist $k$ pairwise internally vertex-disjoint $s$-$t$ paths of length at most $\ell$. The problem has been proven to be NP-hard and fixed-parameter tractable parameterized by $k$ and $\ell$. Most previous research on this problem has been theoretical with limited practical implemetations. We present an exact FPT-algorithm based on a search-tree approach in combination with greedy localization. While its worst case runtime complexity of $(k\cdot \ell^2)^{k\cdot \ell}\cdot n^{O(1)}$ is larger than the state of the art, the nature of search-tree algorithms allows for a broad range of potential optimizations. We exploit this potential by presenting techniques for input preprocessing, early detection of trivial and infeasible instances, and strategic selection of promising subproblems. Those approaches were implemented and heavily tested on a large dataset of diverse graphs. The results show that our heuristic improvements are very effective and that for the majority of instances, we can achieve fast runtimes.

==> tables/h2_False_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h2n', 'h1t', 'h2t',
       'h2\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h2_False_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h2n', 'h1t', 'h2t',
       'h2\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h2_True_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h2n', 'h1t', 'h2t',
       'h2\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h2_True_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h2n', 'h1t', 'h2t',
       'h2\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h2_no_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
instance &    s &   t &  k &  ell & success &  h1n &  h2n &  h1t &   h2t &  h2\_diff \\
\midrule
  fvs056 &  735 & 739 &  5 &    6 &      no &    4 &  655 & 1577 & 10947 &     5.94 \\
  fvs097 &   81 &  53 &  4 &    5 &      no &    5 &  171 &  272 &  1671 &     5.14 \\
  fvs052 & 1586 & 404 &  4 &    7 &      no &   38 &  648 & 2636 & 12384 &     3.70 \\
  fvs100 &   91 &  25 &  5 &    6 &      no &    1 &    1 &   14 &    38 &     1.71 \\
  fvs097 &   89 &  31 &  6 &    6 &      no &    1 &    1 &   13 &    32 &     1.46 \\
\bottomrule
\end{tabular}


==> tables/h2_no_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
 instance &    s &    t &  k &  ell & success &  h1n &  h2n &   h1t &  h2t &  h2\_diff \\
\midrule
   fvs080 &   84 &  105 &  2 &    5 &      no & 2074 &  629 & 31526 & 9444 &    -0.70 \\
planar350 &   40 &   32 &  3 &    7 &      no & 2750 &  953 &  3653 & 1756 &    -0.52 \\
   fvs001 & 4264 & 3660 &  2 &    5 &      no &    9 &    9 &   304 &  148 &    -0.51 \\
      hex &  280 &  230 &  4 &    5 &      no & 4419 &  622 & 10272 & 5006 &    -0.51 \\
planar500 &   44 &  489 &  2 &    8 &      no &    0 &    0 &    16 &   10 &    -0.38 \\
\bottomrule
\end{tabular}


==> tables/h2_yes_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
instance &   s &   t &  k &  ell & success &  h1n &    h2n &  h1t &    h2t &  h2\_diff \\
\midrule
polbooks &  26 &  64 &  7 &    8 &     yes &  289 & 130956 & 1778 & 300001 &   167.73 \\
  fvs047 &  60 &  68 &  4 &    8 &     yes &    4 &     89 &   14 &    155 &    10.07 \\
 sb-10-2 & 387 & 342 &  5 &    6 &     yes &    4 &     66 &  261 &   1282 &     3.91 \\
 cl-10-2 & 405 & 994 &  7 &    5 &     yes &  405 &   1347 & 1246 &   4637 &     2.72 \\
airlines &  51 & 175 &  5 &    8 &     yes &    4 &     24 &  263 &    591 &     1.25 \\
\bottomrule
\end{tabular}


==> tables/h2_yes_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
     instance &  s &   t &  k &  ell & success &    h1n &   h2n &    h1t &   h2t &  h2\_diff \\
\midrule
lesmiserables & 23 &  61 &  5 &    7 &     yes & 207776 &    58 & 172299 &   194 &    -1.00 \\
       karate & 26 &  20 &  3 &    7 &     yes &  58959 &   676 & 110457 &  3406 &    -0.97 \\
     clh-10-0 & 86 &  75 &  5 &    6 &     yes & 423137 & 18317 & 240965 & 21379 &    -0.91 \\
       fvs100 &  6 & 182 &  4 &    7 &     yes &  12892 &  1040 &   4438 &   618 &    -0.86 \\
     dolphins & 10 &  57 &  4 &    6 &     yes & 188715 & 19555 &  95996 & 15998 &    -0.83 \\
\bottomrule
\end{tabular}


==> tables/h3_False_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h3n', 'h1t', 'h3t',
       'h3\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h3_False_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h3n', 'h1t', 'h3t',
       'h3\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h3_True_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h3n', 'h1t', 'h3t',
       'h3\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h3_True_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h3n', 'h1t', 'h3t',
       'h3\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h3_no_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
        instance &   s &   t &  k &  ell & success &  h1n &    h3n &  h1t &    h3t &  h3\_diff \\
\midrule
       planar302 & 167 & 170 &  3 &    7 &      no &    0 & 173799 &    4 & 300005 & 75000.25 \\
          fvs100 &  45 &  37 &  4 &    5 &      no &    0 & 496121 &    7 & 300001 & 42856.29 \\
          fvs047 &  41 &  15 &  4 &    7 &      no &    1 & 219456 &    2 &  68933 & 34465.50 \\
       planar500 &  44 & 489 &  2 &    8 &      no &    0 & 202094 &   16 & 300003 & 18749.19 \\
photoviz\_dynamic &  84 &  88 &  5 &    7 &      no &    4 & 503417 &   40 & 300001 &  7499.02 \\
\bottomrule
\end{tabular}


==> tables/h3_no_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
  instance &    s &   t &  k &  ell & success &  h1n &  h3n &   h1t &  h3t &  h3\_diff \\
\midrule
    fvs097 &   81 &  53 &  4 &    5 &      no &    5 &    1 &   272 &    5 &    -0.98 \\
netscience &  302 & 310 &  2 &    6 &      no &  695 &  818 &  5481 &  853 &    -0.84 \\
    fvs080 &   84 & 105 &  2 &    5 &      no & 2074 &  306 & 31526 & 6825 &    -0.78 \\
    fvs056 & 1596 & 420 &  2 &    7 &      no &    2 & 2857 &  2129 & 1006 &    -0.53 \\
    fvs100 &   91 &  25 &  5 &    6 &      no &    1 &    1 &    14 &    8 &    -0.43 \\
\bottomrule
\end{tabular}


==> tables/h3_yes_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
     instance &  s &  t &  k &  ell & success &  h1n &    h3n &  h1t &    h3t &  h3\_diff \\
\midrule
     dolphins & 40 &  6 &  4 &    8 &     yes &    0 & 163668 &    2 &  87554 & 43776.00 \\
     dolphins & 40 &  6 &  4 &    9 &     yes &    1 & 501978 &    7 & 252118 & 36015.86 \\
lesmiserables & 66 & 49 &  5 &    8 &     yes &    2 & 613161 &   14 & 300003 & 21427.79 \\
lesmiserables & 66 & 51 &  5 &    7 &     yes &    1 & 459061 &   18 & 300001 & 16665.72 \\
    planar400 & 12 & 31 &  3 &    8 &     yes &    1 &    760 &    3 &   1726 &   574.33 \\
\bottomrule
\end{tabular}


==> tables/h3_yes_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
     instance &   s &   t &  k &  ell & success &    h1n &  h3n &    h1t &  h3t &  h3\_diff \\
\midrule
       karate &  26 &  20 &  3 &    7 &     yes &  58959 &    1 & 110457 &    3 &    -1.00 \\
lesmiserables &  23 &  61 &  5 &    7 &     yes & 207776 &    2 & 172299 &   11 &    -1.00 \\
     airlines & 128 & 179 &  4 &    5 &     yes &   7718 &    1 & 110570 &   36 &    -1.00 \\
    planar400 & 348 &  49 &  2 &    8 &     yes &  51861 &   31 & 113134 &   72 &    -1.00 \\
      sb-10-1 & 483 & 801 &  4 &    8 &     yes & 134026 &    1 & 118919 &  147 &    -1.00 \\
\bottomrule
\end{tabular}


==> tables/h4_False_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h4n', 'h1t', 'h4t',
       'h4\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h4_False_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h4n', 'h1t', 'h4t',
       'h4\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h4_True_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h4n', 'h1t', 'h4t',
       'h4\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h4_True_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
Empty DataFrame
Columns: Index(['instance', 's', 't', 'k', 'ell', 'success', 'h1n', 'h4n', 'h1t', 'h4t',
       'h4\_diff'],
      dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}


==> tables/h4_no_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
        instance &   s &   t &  k &  ell & success &  h1n &    h4n &  h1t &    h4t &  h4\_diff \\
\midrule
       planar302 & 167 & 170 &  3 &    7 &      no &    0 &  51464 &    4 & 100387 & 25095.75 \\
          fvs100 &  45 &  37 &  4 &    5 &      no &    0 &  81903 &    7 &  54442 &  7776.43 \\
photoviz\_dynamic &  84 &  88 &  5 &    7 &      no &    4 & 464055 &   40 & 287634 &  7189.85 \\
       planar500 &  44 & 489 &  2 &    8 &      no &    0 &  68285 &   16 & 108286 &  6766.88 \\
          fvs047 &  41 &  15 &  4 &    7 &      no &    1 &  11022 &    2 &   3789 &  1893.50 \\
\bottomrule
\end{tabular}


==> tables/h4_no_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
  instance &    s &   t &  k &  ell & success &  h1n &  h4n &   h1t &  h4t &  h4\_diff \\
\midrule
    fvs097 &   81 &  53 &  4 &    5 &      no &    5 &    1 &   272 &    4 &    -0.99 \\
netscience &  302 & 310 &  2 &    6 &      no &  695 &  251 &  5481 &  297 &    -0.95 \\
       hex &  280 & 230 &  4 &    5 &      no & 4419 & 3825 & 10272 &  988 &    -0.90 \\
    fvs080 &   84 & 105 &  2 &    5 &      no & 2074 &  165 & 31526 & 3855 &    -0.88 \\
    fvs056 & 1596 & 420 &  2 &    7 &      no &    2 &  947 &  2129 &  342 &    -0.84 \\
\bottomrule
\end{tabular}


==> tables/h4_yes_bot.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
     instance &  s &  t &  k &  ell & success &  h1n &    h4n &  h1t &    h4t &  h4\_diff \\
\midrule
lesmiserables & 66 & 49 &  5 &    8 &     yes &    2 & 416483 &   14 & 293510 & 20964.00 \\
     dolphins & 40 &  6 &  4 &    9 &     yes &    1 & 131333 &    7 &  67526 &  9645.57 \\
     dolphins & 40 &  6 &  4 &    8 &     yes &    0 &  33924 &    2 &  19184 &  9591.00 \\
lesmiserables & 66 & 51 &  5 &    7 &     yes &    1 & 209480 &   18 & 170423 &  9466.94 \\
    planar400 & 12 & 31 &  3 &    8 &     yes &    1 &    244 &    3 &    647 &   214.67 \\
\bottomrule
\end{tabular}


==> tables/h4_yes_top.tex <==
\begin{tabular}{lrrrrlrrrrr}
\toprule
     instance &   s &   t &  k &  ell & success &    h1n &  h4n &    h1t &  h4t &  h4\_diff \\
\midrule
       karate &  26 &  20 &  3 &    7 &     yes &  58959 &    1 & 110457 &    3 &    -1.00 \\
lesmiserables &  23 &  61 &  5 &    7 &     yes & 207776 &    2 & 172299 &   11 &    -1.00 \\
     airlines & 128 & 179 &  4 &    5 &     yes &   7718 &    1 & 110570 &   36 &    -1.00 \\
    planar400 & 348 &  49 &  2 &    8 &     yes &  51861 &   31 & 113134 &   98 &    -1.00 \\
      sb-10-1 & 483 & 801 &  4 &    8 &     yes & 134026 &    1 & 118919 &  153 &    -1.00 \\
\bottomrule
\end{tabular}

